Towards Verifying Exact Conditions for Implementations of Density Functional Approximations

Density Functional Theory (DFT) is used extensively in the computation of electronic properties of matter, with various applications. Approximating the exchange-correlation (XC) functional is the key to the Kohn-Sham DFT approach, the basis of most DFT calculations. The choice of this density functional approximation (DFA) depends crucially on the particular system under study, which has resulted in the development of hundreds of DFAs. Though the exact density functional is not known, researchers have discovered analytical properties of this exact functional. Furthermore, these exact conditions are used when designing DFAs. We present XCVerifier, the first approach for verifying whether a DFA implementation satisfies the DFT exact conditions. XCVerifier was evaluated on five DFAs from the popular Libxc library and seven exact conditions from recent work. XCVerifier was able to verify or find violations for a majority of the DFA/condition pairs, demonstrating the feasibility of using formal methods to verify DFA implementations.

==> dft-preliminaries.tex <==
\section{DFT Preliminaries}
\label{sec:DFTPreliminaries}

\meta{DFAs: list and cite the ones we actually verify. } 

\meta{Exact Conditions on functional. Local condition on the function used in the functional.}

\meta{Plot some of the functionals. }

This section presents a brief overview of Density Functional Theory (DFT) and
Density Functional Approximations (DFAs), and provides background on the
analytical and numerical properties of DFAs. More details can be found in
standard reference texts~\cite{engel2011density,koch2015chemist}.

\subsection{Key ideas in DFT}
\label{sec:DFTPreliminaries-KeyIdeas}
Traditional quantum mechanics describes a system of $N$ electrons in terms of a
complex-valued, antisymmetric wave function that depends on the coordinates of each
electron, i.e.\ a function of $3N$ variables that must satisfy the \schrodinger\
equation. Solving the \schrodinger\ equation becomes intractable for systems
including more than a few electrons. 
DFT shifts focus to the electron density, a real function
representing the electron probability distribution in three-dimensional space.

The Hohenberg-Kohn Theorem serves as the cornerstone of DFT.
This theorem proves that the ground-state energy of a system is uniquely
determined by its electron density. This implies that all other ground-state
properties can also be derived from the density, eliminating the need for wave
functions.

The Kohn-Sham (KS)~\cite{kohn1965self} approach is currently the basis of most DFT calculations.

\subsection{Density Functional Approximations} 
\label{sec:DFTPreliminaries-DFA}

Assuming the KS form of kinetic energy approximation, an energy functional still
lacks an exact expression for the exchange-correlation energy of a density 
$n(r)$ (\meta{or $\rho(r)$}). This exchange-correlation energy, $E_{XC}$, is
a universal but unknown function of $n(r)$~\cite{ZIESCHE1998122}.

Local density approximations (LDA)~\cite{kohn1965self}, 
were the first class of DFAs created to approximate $E_{XC}$.
They depend only on the electron density $n(r)$ (\meta{$\rho(r)$}) (Equation~\ref{eq:lda}).
\begin{equation*}
    E_{XC}^{LDA} = \int n(r) \epsilon_X^{LDA}(n(r)) dr
    \label{eq:lda}
\end{equation*}

The mathematical expression for the exchange part $\epsilon_X$ of an LDA
functional from \libxc{} is shown in Equation~\ref{eq:lda}. 
~\meta{LDA functional vs LDA class of functionals is confusing. Maybe use VWN as an example.}

\begin{equation*}
\epsilon^{LDA}_X = 2.0 \left(\begin{cases} 0 & \text{for}\: \rho \leq 0 \\- 0.369279383191011
\rho^{1/3} & \text{otherwise} \end{cases}\right)
\label{eq:lda_exchange}
\end{equation*}

Generalized Gradient Approximations (GGAs)~\cite{perdewandwang1991ggas} depend
on the electron density and its gradient 
GGA functionals improve upon LDA functionals (\meta{and local spin density
approximation (LSDA) functionals--similar to LDA and include the spin
polarization}) are often used in practice~\cite{perdew1996generalized}. In
addition to the electron density, they also depend on the gradient of the
electron density $\sigma$ (Equation~\ref{eq:gga}).

\begin{equation*}
    E_{XC}^{GGA} = \int n(r) \epsilon_X^{GGA}(n(r), \nabla n(r)) dr
    \label{eq:gga}
\end{equation*}

The Perdew-Burke-Ernzerhof (PBE) functional~\cite{perdew1996generalized} is a
popular GGA functional and commonly used in practice~\cite{2009whichshouldichoose}.
The equation for the exchange part is shown in
Equation~\ref{eq:pbe_exchange}. 
\begin{equation*}
    \epsilon^{PBE}_X = \frac{2.884 \rho^{1/3} \left(- 28.944 \pi^{4/3} \rho^{8/3} - 0.174 \pi^{2} \sigma\right)}{\pi^{1/3} \cdot \left(77.184 \pi^{4/3} \rho^{8/3} + 0.257 \pi^{2} \sigma\right)}
    \label{eq:pbe_exchange}
\end{equation*}

However, the correlation part of PBE is significantly more complex with over 300
operations according to Sympy. The strongly constrained and appropriately normed
(SCAN) functional, a meta-GGA functional designed to satisfy the 17 constraints
and norms~\cite{sun2015scan}, is even more complex with over 1000 operations in the exchange and
correlation parts combined.


\subsection{Exact Conditions of DFAs}
\label{sec:DFTPreliminaries-ExactConditions}

We list seven exact conditions of interest from~\cite{Pederson2023} and their local counterparts. 
We check the satisfiability of the exact conditions for the DFAs via the local 
conditions \meta{why}.
Where the exact conditions take as input the global energy $\exc[n(r)]$ of the DFA, the 
local conditions take the exchange (correlation) enhancement factor $\fxc$, which is a function of 
the local value $\epsxc(n(r))$ of the exchange (correlation) energy of the DFA.

We can express the inputs to a DFA, $n(r),\nabla n$, in terms of the Wigner-Seitz radius
$r_s=(r\pi n/3)^{-1/3}$ and $s=|\nabla n|/(2(3\pi^2)^{1/3}n^{4/3})$.
Given the expressions for the exchange and correlation energies
$\epsxtilde$ and $\epsctilde$ of the DFA in terms of $s$ and $r_s$, we can 
compute $\fc$ and $\fc$ of $\fxc$: 
\begin{equation}
    \fxc[n(r)] = \fx + \fc = \frac{\tilde{\epsilon}_{X(C)}[n(r)]}{\epsilon_X^{\text{unif}}[n(r)]},
\end{equation}
\changed{
where ${\epsilon_X^{\text{unif}}[n(r)]}=-(3/4\pi)(3\pi^2n)^{1/3}$ is the exchange energy per particle of an unpolarized 
electron gas with uniform density $n(r)$~\cite{KURTH2005395}.
}

As discussed e.g.\ by Pederson and Burke~\cite{pederson2023difference},
constraints on the global energy can be enforced by imposing the
same constraint locally, although it is considered in some cases to
be too stringent as most ``reasonable'' densities---originating from actual molecules---may
violate the local constraint while obeying the global one. 

\subsubsection{Exact and Local Conditions}
\begin{itemize}
    \item The correlation energy $E_C$ non-positivity
    condition~\cite{Pederson2023} (\meta{holds for any reasonable density}) is 
    \begin{equation}
        E_C[n] \leq 0.
    \end{equation}
    The corresponding local condition is
    \begin{equation}
        \epsilon_C[n(r)] \leq 0. %
        \label{eq:local-ec}
    \end{equation}
    
    \item The $E_C$ scaling inequality~\cite{PhysRevA.32.2010,Pederson2023},
    \begin{equation}
        (\gamma-1)E_C[n_\gamma] \geq \gamma(\gamma - 1) E_C[n],
    \end{equation}
    has the local condition
    \begin{equation}
        \frac{\partial \fc}{\partial r_s} \geq 0. %
        \label{eq:local-ec-scaling}
    \end{equation}
    
    \item The $\uc(\lambda)$ monotonicity condition~\cite{PhysRevB.48.11638,Pederson2023},
    where $\uc(\lambda) = d(\lambda^2E_C[n_{1/\lambda}])/d\lambda$ represents
    the correlation energy adiabatic connection curves, is 
    \begin{equation}
        \frac{d\uc(\lambda)}{d\lambda} \leq 0,
    \end{equation}
    The corresponding local condition is
    \begin{equation}
        \frac{\partial}{\partial r_s}\left(r_s^2\frac{\partial \fc}{\partial r_s}\right) \geq 0,
    \end{equation}
    which is rewritten as 
    \begin{equation}
        \frac{\partial^2 F_c}{\partial r_s^2} \geq \frac{-2}{r_s} \cdot \frac{\partial F_c}{\partial r_s}.
        \label{eq:local-uc}
    \end{equation}

    \item Lieb-Oxford bound~\cite{https://doi.org/10.1002/qua.560190306,Pederson2023} is
    \begin{equation}
        U_{XC} \geq C_{LO}\int d^3 r\, n\, \epsilon_{X}^{\text{unif}}[n(r)].
    \end{equation}
    where $U_{XC}[n] = E_{XC}[n] - \tc[n]$ is the potential correlation energy. The corresponding local condition is
    \begin{equation}
        \fxc + r_s\frac{\partial \fc}{\partial r_s} \leq C_{LO}.
        \label{eq:local-lo}
    \end{equation}
    where $C_{LO}=2.27$ is the Lieb-Oxford constant, following~\cite{Pederson2023}. Tighter bounds have been proven~\cite{Lewin2019,Lewin2022}

    \item The Lieb-Oxford extension to $E_{XC}$~\cite{https://doi.org/10.1002/qua.560190306,Pederson2023} is
    a generalization of the Lieb-Oxford bound with $E_{XC}$ instead of $U_{XC}$:
    \begin{equation}
        E_{XC} \geq C_{LO}\int d^3 r\, n\, \epsilon_{X}^{\text{unif}}[n(r)].
    \end{equation}
    The corresponding local condition is
    \begin{equation}
       \fxc \leq C_{LO}
       \label{eq:local-lo-exc}
    \end{equation}

    \item The $\tc$ upper bound condition~\cite{PhysRevB.48.11638,Pederson2023} is
    \begin{equation}
        \tc[n_\gamma] \leq -\gamma \left(\frac{\partial E_C[n_\gamma]}{\partial\gamma}\right) + E_C[n_\gamma].
    \end{equation}
    The corresponding local condition is
    \begin{equation}
        \frac{\partial \fc}{\partial r_s} \leq \frac{\fc(\infty) - \fc}{r_s}.
        \label{eq:local-tc}
    \end{equation}    
    where $\fc(\infty)$ is the limit of $\fc$ as $r_s \to \infty$.

    \item The \emph{conjectured} $\tc$ upper bound~\cite{Levy1985,10.1063/1.481099,Crisostomo2023,Pederson2023} is
    \begin{equation}
        \tc[n] \leq -E_C[n]
    \end{equation}
    with local condition
    \begin{equation}
        \frac{\partial \fc}{\partial r_s} \leq \frac{\fc}{r_s}.
        \label{eq:local-tc-conjectured}
    \end{equation}
\end{itemize}

\subsection{Satisfiability Modulo Theory (SMT) Solvers}
SMT is the problem of determining the satisfiability of a mathematical formula.
Efficient algorithms exist for solving SMT problems with only linear arithmetic.
In general, non-linear SMT problems are undecidable.

\meta{Insert a brief explanation of SMT solvers.}
\subsubsection{dReal}
The \dreal{} SMT solver~\cite{gao2013dreal} supports non-linear real arithmetic (NRA)
and can handle several analytical functions.
Given a formula $\phi$ in the logic of non-linear real arithmetic, 
such SMT solvers are able determine whether or not there exists a satisfying assignment to $\phi$; 
that is, if there is any assignment to the variables in $\phi$ that makes the formula evaluate to True. 
Moreover, the solvers are able to compute such a satisfying assignment, if it exists. 

\dreal{} implements a delta-complete decision framework. Given a formula $\varphi$,
instead of return \UNSAT{} ($\varphi$ is unsatisfiable) or \SAT{} ($\varphi$ is
satisfiable for the returned model), dReal returns \UNSAT{} or $\delta$-\SAT{} (the
$\delta$-weakening $\varphi^{\delta}$ is satisfiable for the returned model).
The $\delta$-weakening $\varphi^{\delta}$ of a formula $\varphi$ is numerical
relaxation of $\varphi$. \meta{A model that satisfies $\varphi$ will always
satisfy $\varphi^{\delta}$, however, the reverse is not necessarily true. If
$\varphi^{\delta}$ is unsatisfiable then $\varphi$ is also unsatisfiable.}

This relaxation results dReal now being decidable for nonlinear formulas.
That is, the bounded $\delta$-SMT problem is decidable for many nonlinear formulas,
including those with transcendental functions, which are common in DFAs.



==> overview.tex <==
\section{Overview}
\label{sec:Overview}

\meta{Provide a walkthrough of the solution by going through an example. This
section should give a high-level description of the techniques, and provide
insights on the solution.}



==> preliminaries.tex <==
\section{Preliminaries}
\label{sec:Preliminaries}


==> problem-statement.tex <==
\section{Problem Statement}
\label{sec:ProblemStatement}


DFAs are typically designed to satisfy a number of constraints that derive from known 
results about specific physical systems. The most commonly used system is the homogeneous
electron gas (HEG) which consists of an infinite system of constant electronic density.
All non-empirical DFAs are required to describe the HEG exchange-correlation energy correctly.
This constraint is typically enforced by adopting a local representation of the exchange-correlation
energy density $\epsilonxc(n(r),|\nabla n(r)|)$ that trivially reduces to the appropriate value
when $n(r)$ is constant and $\nabla n(r)$ vanishes. Various other constraints imposed on 
$\epsilonxc$ affect specific parts of its definition. An example is the
Lieb-Oxford bound~\cite{lieb1981improved} which is often used to limit values of the so-called
exchange energy enhancement factor found in many DFAs.
Other DFAs (referred to as empirical) make use of adjusted parameters that make them reproduce the 
results of high-accuracy quantum chemistry calculations involving wave functions of specific molecular
benchmarks. 
Empirical DFAs typically do not satisfy the same constraints that non-empirical DFAs enforce, 
and might violate these constraints in some regions of the input space. 
Thus, understanding when a given DFA satisfies a given physical constraint would be helpful 
in explaining the behavior of existing DFAs. 

This motivates the following problem of \emph{DFA Exact-Condition Analysis}: 
\begin{mdframed} 
Input: DFA $\exc$, exact condition $\psi$ (defined using non-linear \emph{real} arithmetic) \\
Output: input region represented by $\varphi$ 
such that $\exc$ satisfies $\psi$ in the input region $\varphi$. 
\end{mdframed}


